A Fast, Simple, Robust Algorithm for Coronal Temperature Reconstruction

We describe a new algorithm for reconstruction of Differential Emission Measures (DEMs) in the solar corona. Although a number of such algorithms currently exist, they can have difficulty converging for some cases, and can be complex, slow, or idiosyncratic in their output (i.e., their inversions can have features that are a result of the inversion code and instrument response, not of the solar source); we will document some of these issues in this paper. The new algorithm described here significantly reduces these drawbacks and is particularly notable for its simplicity; it is reproduced here, in full, on a single page. After we describe the algorithm, we compare its performance and fidelity with some prevalent methods. Although presented here for extreme ultraviolet (EUV) data, the algorithm is robust and extensible to any other wavelengths (e.g., X-rays) where the DEM treatment is valid.

==> aastex_journals.tex <==
%AASTEX journal commands
%Copied from version 5.2 (2005) by D. C. Jacobs 2008

\let\jnlatstyle=\rmfamily
\def\refatjnl#1{{\jnlatstyle#1}}%
\newcommand\aj{\refatjnl{AJ}}%
          % Astronomical Journal
\newcommand\actaa{\refatjnl{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{\refatjnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\refatjnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\refatjnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\refatjnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\refatjnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\refatjnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\refatjnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\refatjnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\refatjnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\refatjnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\refatjnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{\refatjnl{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\refatjnl{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\refatjnl{Icarus}}%
  % Icarus
\newcommand\jcap{\refatjnl{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\refatjnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\refatjnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\refatjnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{\refatjnl{New A}}%
  % New Astronomy
\newcommand\nar{\refatjnl{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{\refatjnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\refatjnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\refatjnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\refatjnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\refatjnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\refatjnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{\refatjnl{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\refatjnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\refatjnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\refatjnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\refatjnl{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\refatjnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\refatjnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\refatjnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\refatjnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\refatjnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\refatjnl{Nature}}%
          % Nature
\newcommand\iaucirc{\refatjnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\refatjnl{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\refatjnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\refatjnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\refatjnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\refatjnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\refatjnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\refatjnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\refatjnl{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\refatjnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\refatjnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\refatjnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\refatjnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\refatjnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\refatjnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\refatjnl{Proc.~SPIE}}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

